When, Why, and Which Pretrained GANs Are Useful?

The literature has proposed several methods to finetune pretrained GANs on new datasets, which typically results in higher performance compared to training from scratch, especially in the limited-data regime. However, despite the apparent empirical benefits of GAN pretraining, its inner mechanisms were not analyzed in-depth, and understanding of its role is not entirely clear. Moreover, the essential practical details, e.g., selecting a proper pretrained GAN checkpoint, currently do not have rigorous grounding and are typically determined by trial and error. This work aims to dissect the process of GAN finetuning. First, we show that initializing the GAN training process by a pretrained checkpoint primarily affects the model's coverage rather than the fidelity of individual samples. Second, we explicitly describe how pretrained generators and discriminators contribute to the finetuning process and explain the previous evidence on the importance of pretraining both of them. Finally, as an immediate practical benefit of our analysis, we describe a simple recipe to choose an appropriate GAN checkpoint that is the most suitable for finetuning to a particular target task. Importantly, for most of the target tasks, Imagenet-pretrained GAN, despite having poor visual quality, appears to be an excellent starting point for finetuning, resembling the typical pretraining scenario of discriminative computer vision models.

==> related.tex <==
\section{Related Work}
\label{sect:related}




==> toy_example/sngan.tex <==
\textbf{MNIST.} As for the extension of the synthetic data GAN transfer analysis to the real data, we consider the Spectral Norm GAN \citep{miyato2018spectral} with the transfer task from Omniglot \citep{omniglot} as a source data to MNIST \citep{lecun2010mnist} as a target data. All training and architectural details are provided in the supplementary. Our aim is to show the superiority of the gradients provided by a pretrained discriminator on a source domain to the random initialization. Similar to the synthetic data experiment, we form a ground truth vector field of a generator guidance and evaluate its cosine similarity with the gradients field provided by the discriminator. First, as for the ground truth direction for a generated sample $G(z)$ with an Omniglot-pretrained generator, we take the $l_2$-closest MNIST sample $x$. In purpose to increase spatial invariance, we always operate with the images downscaled to $16\times 16$. As for the referral gradient field, we take the direction to the closest target sample $x - G(z)$. The average cosine similarity between the Omniglot-pretrained discriminator gradients field and the referral vector field is equal $0.146$. As for averaging we always take 1000 randomly generated samples. Given the same samples, the averaged cosine similarity between a randomly initialized discriminator and the referral vector field is equal $-0.04$ with the standard deviation $0.07$. Here we report the value averaged over 10 independent random discriminator initializations. This confirms the superiority of a pretrained discriminator gradients field to the random initialization.
